Database Learning: Toward a Database that Becomes Smarter Every Time

In today's databases, previous query answers rarely benefit answering future queries. For the first time, to the best of our knowledge, we change this paradigm in an approximate query processing (AQP) context. We make the following observation: the answer to each query reveals some degree of knowledge about the answer to another query because their answers stem from the same underlying distribution that has produced the entire dataset. Exploiting and refining this knowledge should allow us to answer queries more analytically, rather than by reading enormous amounts of raw data. Also, processing more queries should continuously enhance our knowledge of the underlying distribution, and hence lead to increasingly faster response times for future queries. We call this novel idea---learning from past query answers---Database Learning. We exploit the principle of maximum entropy to produce answers, which are in expectation guaranteed to be more accurate than existing sample-based approximations. Empowered by this idea, we build a query engine on top of Spark SQL, called Verdict. We conduct extensive experiments on real-world query traces from a large customer of a major database vendor. Our results demonstrate that Verdict supports 73.7% of these queries, speeding them up by up to 23.0x for the same accuracy level compared to existing AQP systems.

==> correlation_learning.tex <==

%\input{fig_exp_correlation_new}



\subsection{Accuracy of Parameter Learning}
\label{sec:exp:correlation}

In this section, we examine the effectiveness of \dbl's correlation parameter estimation process
presented in \cref{sec:learn}. Similar to \cref{sec:exp:validation}, we used the synthetic datasets
generated from pre-determined correlation parameters to see how close \dbl could estimate the values
of those correlation parameters. We let \dbl estimate the correlation parameter values using three
different numbers of past snippets (20, 50, and 100) for various datasets with different
correlation parameter values.

\input{fig_exp_correlation_learning}

\Cref{fig:param_learning} shows the results. In general, the correlation parameter values discovered
by \dbl's estimation process were consistent with the true correlation parameter values. Also, the
estimated values tended to be closer to the true values when a larger number of past snippets were
used for the estimation process. This result indicates that \dbl can effectively learn statistical
characteristics of the underlying distribution just based on the answers to the past queries.




==> cov.tex <==
\section{Covariance Computation}
\label{sec:cov}

This section in interested in analytically calculating the following expression:
\[
\int_a^b \int_c^d
 \exp \left( -\frac{(x_1 - x_2)^2}{2 l^2} \right) \; d x_1 d x_2.
\]
The result of the above double integral calculation can be applied directly to obtain the result of Expression~\ref{eq:cov} if $g_{A_1}(a_1)$ and $g_{A_1}(a'_1)$ are uniform within the range $(l^{(i)}, u^{(i)})$ and $(l^{(j)}, u^{(j)})$ respectively. If $g_{A_1}(a_1)$ and $g_{A_1}(a'_1)$ are not uniform and are available as histograms, one can break the integral expression into subranges within which pdf is uniform, then combine their results.

The computation of the double integral above relies on the following two facts~\cite{ng1969table}:
\begin{align*}
  \int_0^x e^{-t^2} \; dt &= \frac{\sqrt{\pi}}{2} \erf(x) \\
  \int_0^x \erf(at) \; dt &= x \erf(ax)
   + \frac{1}{a \sqrt{\pi}} \left( \exp(-a^2 x^2) - 1 \right)
\end{align*}
where $\erf(x)$ is an error function.


==> covariance_tech.tex <==
\section{Details on Computing Covariances Between Query Answers}
\label{sec:appendix:cov}

Let  $g$  be an aggregate function on attribute $A_k$, 
$\rcol_k$ be a random variable representing  the possible values of
attribute $A_k$, 
$\mtuple = (a_1, \ldots, a_l)$ be a vector of length $l$ comprised of values for $r$'s
dimension attributes   $A_1, \ldots, A_l$, and $\omega(\mtuple)$ be  the fraction of tuples in $r$ that have the same  values for their 
dimension attributes as $\mtuple$.

We use $\nu_g(\mtuple)$ to denote the expected value of aggregate function $g$ given the values of dimension attributes.
Thus, we have:
\begin{align*}
  \nu_g(\mtuple) = \begin{cases}
    E[\rcol_k \mid \mtuple]  & \qquad \text{if $g$ is \texttt{AVG($A_k$)}} \\
    \omega(\mtuple)    & \qquad \text{if $g$ is \texttt{FREQ(*)}}
  \end{cases}
\end{align*}
Therefore, $\nu_g(\mtuple)$ is a random variable dependent on
$\mtuple$ (since relation $r$ is drawn from an underlying
distribution).

Let $\filter_i$ denote the set of tuples satisfying the
selection predicates of $q_i$. Then, the random variable $\rtans_i$ representing  possible true answers to $q_i$ can be
expressed in terms of $\nu_g(\mtuple)$:
\begin{align}
  \rtans_i =
  \begin{cases}
    \begin{aligned}
      \frac{1}{\mathcal{Z}_i}
      \int_{\filter_i} \nu_g(\mtuple) \, \omega(\mtuple) \; d\mtuple
    \end{aligned}
    & \text{if $g$ is \texttt{AVG($A_k$)}} \\
    \begin{aligned}
      \int_{\filter_i} \nu_g(\mtuple) \; d\mtuple
    \end{aligned}
    & \text{if $g$ is \texttt{FREQ(*)}}
  \end{cases}
  \label{eq:appendix:query_answer}
\end{align}
where $\mathcal{Z}_i$ is a normalization term defined as $\mathcal{Z}_i = \int_{\filter_i} \omega(\mtuple) \; d\mtuple$.
%Also, $E(\rtans_i)$ is equal to
%$\qmean$ because $E(\nu_g(\mtuple))$ is a constant. In practice, \dbl
%determines the value of $\qmean$ by averaging past queries answers.


Based on equation (\ref{eq:appendix:query_answer}), 
the covariance between random variables $\rans_i$ and
$\rans_j$ can be expressed as follows. (This quantity corresponds to the variance of $\rans_i$ if
$i = j$.)
\begin{align}
  & E \left[ (\rans_i - \qmean_i)(\rans_j - \qmean_j) \right]
  = E \left[ (\rtans_i + \rerr_i - \qmean_i)(\rtans_j + \rerr_j - \qmean_j) \right] \nonumber \\
  &=
  \begin{cases}
    \begin{aligned}
      \frac{1}{\mathcal{Z}_i \mathcal{Z}_j}
      \int_{\filter_i} \int_{\filter_j}
      \cov(\nu_g(\mtuple), \nu_g(\mtuple')) \, & \omega(\mtuple) \omega(\mtuple') \, d\mtuple' d\mtuple \\
      \; + \; \delta(i,j) \cdot \beta_i \qquad
      &\text{if $g$ is \texttt{AVG($A_k$)}}
    \end{aligned} \\[2em]
    \begin{aligned}
      \int_{\filter_i} \int_{\filter_j}
      \cov(\nu_g(\mtuple), \nu_g(\mtuple'))
      \, d\mtuple' & d\mtuple \; + \; \delta(i,j) \cdot \beta_i \\
      & \quad \text{if $g$ is \texttt{FREQ(*)}}
    \end{aligned}
  \end{cases}
  \label{eq:appendix:query_cov}
\end{align}
where $\delta$ is 1 if $i = j$ and 0 otherwise; and $\rerr_i$ is a random
variable with variance $\beta_i$ representing 
the deviation of the raw answer from $q_i$'s true
answer.



==> exp_coverage.tex <==
\begin{table}
\centering
\small
\begin{tabular}{|l|l|r|r|}
\hline
Technique          & Constraints & in TPCH & in Vertica \\ \hline
Online Aggregation &   &  &  \\ \hline
Query Column Set   &   &  &  \\ \hline
DB Learning        &   &  &  \\ \hline
\end{tabular}
\caption{Types of queries supported by different techniques and their coverages
of TPC-H and Vertica queries.}
\end{table}


==> exp_improvement.tex <==
\begin{figure*}
\centering

\begin{minipage}[b]{\linewidth}
\begin{subfigure}[b]{0.24\linewidth}

\begin{tikzpicture}
\begin{axis}[
    width=45mm,
    height=45mm,
    xlabel=Approximate Query Latency,
    ylabel=Average Error
]

\end{axis}
\end{tikzpicture}
\caption{Query Set 1}
\end{subfigure}
~
\begin{subfigure}[b]{0.24\linewidth}

\begin{tikzpicture}
\begin{axis}[
    width=45mm,
    height=45mm,
    xlabel=Approximate Query Latency,
    ylabel=Average Error
]

\end{axis}
\end{tikzpicture}
\caption{Query Set 2}
\end{subfigure}
~
\begin{subfigure}[b]{0.24\linewidth}

\begin{tikzpicture}
\begin{axis}[
    width=45mm,
    height=45mm,
    xlabel=Approximate Query Latency,
    ylabel=Average Error
]

\end{axis}
\end{tikzpicture}
\caption{Query Set 3}
\end{subfigure}
~
\begin{subfigure}[b]{0.24\linewidth}

\begin{tikzpicture}
\begin{axis}[
    width=45mm,
    height=45mm,
    xlabel=Approximate Query Latency,
    ylabel=Average Error
]

\end{axis}
\end{tikzpicture}
\caption{Query Set 4}
\end{subfigure}
\end{minipage}

\vspace{4mm}

\begin{minipage}[b]{\linewidth}
\begin{subfigure}[b]{0.24\linewidth}

\begin{tikzpicture}
\begin{axis}[
    width=45mm,
    height=45mm,
    xlabel=Average Error,
    ylabel=Speedup
]

\end{axis}
\end{tikzpicture}
\caption{Query Set 1}
\end{subfigure}
~
\begin{subfigure}[b]{0.24\linewidth}

\begin{tikzpicture}
\begin{axis}[
    width=45mm,
    height=45mm,
    xlabel=Average Error,
    ylabel=Speedup
]

\end{axis}
\end{tikzpicture}
\caption{Query Set 2}
\end{subfigure}
~
\begin{subfigure}[b]{0.24\linewidth}

\begin{tikzpicture}
\begin{axis}[
    width=45mm,
    height=45mm,
    xlabel=Average Error,
    ylabel=Speedup
]

\end{axis}
\end{tikzpicture}
\caption{Query Set 3}
\end{subfigure}
~
\begin{subfigure}[b]{0.24\linewidth}

\begin{tikzpicture}
\begin{axis}[
    width=45mm,
    height=45mm,
    xlabel=Average Error,
    ylabel=Speedup
]

\end{axis}
\end{tikzpicture}
\caption{Query Set 4}
\end{subfigure}
\end{minipage}

\caption{Error Reduction and Speedup of our system.}
\end{figure*}


==> exp_model_validate.tex <==

\subsection{Effect of Model Validation}
\label{sec:exp:validation}

This section studies the effect of \dbl's model validation described in \cref{sec:safeguard}. For
this study, we first generated synthetic datasets with several predetermined correlation parameters
values.
Note that one can generate such synthetic datasets by first determining a joint probabilistic
distribution function with predetermined correlation parameter values and sampling attribute values from the
joint probability distribution function. In usual usage scenario, \dbl estimates those correlation
parameters from past snippets; however, in this section, we manually set the values for the
correlation parameters in \dbl's model, to test the behavior of \dbl running with possibly incorrect
correlation parameter values.

\input{fig_exp_model_validation}

\Cref{fig:model_validation} report the experiment results when \dbl was tested without a model
validation step and with a model validation step, respectively. In the figure, the value on the X-axis
indicates the value multiplied to the true correlation parameters before setting the values in
\dbl's model. For instance, if a true correlation parameter was 5.0, and ``artificial correlation
parameter scale'' was 0.2, \dbl's model was set 1.0 for the correlation parameter. Thus, the values of
correlation parameters were the same as the true correlation parameters when ``artificial correlation
parameter scale'' was 1.0. Since the Y-axis is reporting the ratio of the actual error to \dbl's error
bound, \dbl's error bound was correct when the value on the Y-axis is below 1.0.

In the figure, one can observe that, \dbl used without the model validation produced incorrect error
bounds when the correlation parameters used for the model deviated largely from the true correlation
parameter values.
However, \dbl's model validation could successfully identify incorrect model-based answers and
provide correct error bounds by replacing those incorrect model-based answers with the raw answers
computed by the AQP system.





==> exp_scalability.tex <==
\begin{figure}
\centering

\begin{minipage}[b]{\linewidth}
\begin{subfigure}[b]{0.49\linewidth}
\begin{tikzpicture}
\begin{axis}[
    width=40mm,
    height=40mm,
    xlabel=Spark Node Counts,
    ylabel=Speedup,
]
\end{axis}
\end{tikzpicture}
\end{subfigure}
~
\begin{subfigure}[b]{0.49\linewidth}
\begin{tikzpicture}
\begin{axis}[
    width=40mm,
    height=40mm,
    xlabel=Database Size,
    ylabel=Speedup,
]
\end{axis}
\end{tikzpicture}
\end{subfigure}
\end{minipage}

\caption{Error reduction with different Spark node counts and database size.}
\end{figure}


==> fig_exp_contribution.tex <==
\begin{figure}[t]

  \pgfplotsset{contgraph/.style={
      width=55mm,
      height=28mm,
      xtick={1, 2, 3},
      xticklabels={novel, identical, mixture},
      ytick={0,20,40,60,80,100},
      xmin=0.5,
      xmax=3.5,
      ymin=0,
      ymax=100,
      bar width=5pt,
      %xmode=log,
      xlabel near ticks,
      xlabel shift=-2pt,
      ylabel shift=-2pt,
      xlabel near ticks,
      xlabel style={align=center},
      ylabel=Error\\ Reduction (\%),
      ylabel style={align=center},
      legend style={
        at={(1.1,1)},anchor=north west,column sep=2pt,
        draw=none,font=\scriptsize,fill=none,line width=.5pt,
        /tikz/every even column/.append style={column sep=20pt}
      },
      legend columns=1,
      every axis/.append style={font=\scriptsize},
      ybar=4pt,
      area legend,
      xtick style={draw=none},
      ymajorgrids,
      legend cell align=left,
      %nodes near coords
  }}

  \pgfplotsset{tealbar/.style={
      draw=black!50!darkteal,
      fill=darkteal,
  }}

  \pgfplotsset{graybar/.style={
      draw=black!50!gray,
      fill=gray,
  }}

  \pgfplotsset{redbar/.style={
      draw=black!50!darkorange,
      fill=darkorange,
  }}

  \centering
  \begin{tikzpicture}
    \begin{axis}[contgraph]

      \addplot[tealbar]   % stat error
      table[x=x,y=y]{
        x	y
        1	54.5797361
        2	97.89957114
        3	81.09147515
      };

      \addplot[redbar]   % actual error
      table[x=x,y=y]{
        x	y
        1	51.11931139
        2	96.8188678
        3	79.08743991
      };

      \addlegendentry{stat.~error};
      \addlegendentry{actual error};

    \end{axis}
  \end{tikzpicture}

  \caption{Benefits of correlation modeling. \dbl could improve query answer accuracies even for novel queries.
  Error reductions are reported for a fixed sample size.  Mixture (TPC-H) included 39\% novel queries.}
  \label{fig:exp:contribution}
\end{figure}




==> fig_exp_correlation.tex <==
\begin{figure}[t]
\begin{subfigure}[b]{0.48\linewidth}
  \pgfplotsset{corranal/.style={
      width=45mm,
      height=30mm,
      xmin=0,
      xmax=1,
      ymin=0,
      ymax=1.1,
      %xtick={1, 2, 3, 4, 5, 6},
      %xticklabels={1\%, 2\%, 4\%, 8\%, 16\%, 32\%},
      ytick={0, 0.2, ..., 1.0},
      %bar width=7pt,
      ylabel near ticks,
      ylabel shift=-3pt,
      xlabel near ticks,
      ylabel style={align=center},
      %xmode=log,
      xlabel=True Correlation Parameter,
      ylabel=Learned\\ Corr Param,
      legend style={
        at={(0.2,1)},anchor=south west,column sep=3pt,
        draw=none,font=\scriptsize,fill=none,font=\scriptsize,line width=.5pt,
        /tikz/every even column/.append style={column sep=5pt}
      },
      legend columns=3,
      every axis/.append style={font=\scriptsize},
      %area legend,
      tick style={draw=none},
      legend cell align=left,
      %legend image post style={darkorange,line width=1pt},
  }}

  \pgfplotsset{scatterdots/.style={
      fill=gray,
      draw=none,
      only marks,
      mark size=1.5,
      opacity=0.8,
  }}

  \centering
  \begin{tikzpicture}
    \begin{axis}[corranal]

      \addplot[scatterdots]
      table[x=x,y=y1] {data/cov_analysis.csv};

      \addplot[scatterdots,fill=darkteal]
      table[x=x,y=y2] {data/cov_analysis.csv};

      \addplot[scatterdots,fill=darkorange]
      table[x=x,y=y3] {data/cov_analysis.csv};

      \addplot[draw=black,mark=none] coordinates {(0,0) (1,1)};

      %\addplot[scatterdots,fill=red,draw=black!50!red]
      %table[x=x,y=y4] {data/cov_analysis.csv};

      \addlegendentry{20};
      \addlegendentry{50};
      \addlegendentry{100};
    \end{axis}

    \node[font=\scriptsize] at (-0.2,1.7) {\# past queries:};

  \end{tikzpicture}
  \vspace{-3mm}

  \caption{Correlation Param Learning}
\end{subfigure}
~
\begin{subfigure}[b]{0.48\linewidth}
  \pgfplotsset{paramest/.style={
      width=45mm,
      height=28mm,
      xtick={1, 2, 3, 4, 5, 6, 7, 8},
      xticklabels={-10\%, -5\%, -2\%, -1\%, 1\%, 2\%, 5\%, 10\%},
      ytick={0,5,10,15,20},
      xmin=0.5,
      xmax=8.5,
      ymin=0,
      ymax=20,
      bar width=3pt,
      %xmode=log,
      xlabel near ticks,
      xlabel shift=-4pt,
      ylabel shift=-3pt,
      xlabel near ticks,
      xlabel style={align=center},
      xlabel=Relative Parameter Error (\%),
      ylabel=Conf Interval\\ Violation (\%),
      ylabel style={align=center},
      legend style={
        at={(-0.3,1)},anchor=south west,column sep=2pt,
        draw=none,font=\scriptsize,fill=none,line width=.5pt,
        /tikz/every even column/.append style={column sep=7pt}
      },
      legend columns=2,
      every axis/.append style={font=\scriptsize},
      ybar=1.5pt,
      area legend,
      xtick style={draw=none},
      ymajorgrids,
      legend cell align=left,
      x tick label style={rotate=60, anchor=east,xshift=3pt},
      %nodes near coords
  }}

  \pgfplotsset{tealbar/.style={
      draw=black!50!darkteal,
      fill=darkteal,
  }}

  \pgfplotsset{redbar/.style={
      draw=black!50!darkorange,
      fill=darkorange,
  }}

  \centering
  \begin{tikzpicture}
    \begin{axis}[paramest]

      \addplot[tealbar]   % stat error
      table[x=x,y=y]{
        x	y
        1	10.5
        2	12.6
        3	13.7
        4	8.7
        5	8.7
        6	15.5
        7	8.9
        8	10.8
      };

      \addplot[redbar]   % actual error
      table[x=x,y=y]{
        x	y
        1	1.2
        2	1.0
        3	0.8
        4	0.3
        5	0.0
        6	0.2
        7	1.5
        8	0.2
      };

      \addlegendentry{w/o guard};
      \addlegendentry{w/ guard};

    \end{axis}
  \end{tikzpicture}
  \caption{Under/Over Estimation}
\end{subfigure}

\caption{\tofix{\dbl's correlation learning and its robustness: (a)
the relationship between true correlations and empirically learned correlations,
(b) confidence
interval violations as learned parameter values deviate from the true values.}}
\label{fig:exp:correlation}
\vspace{\neggap}
\end{figure}




==> fig_exp_correlation_full.tex <==
\begin{figure*}[t]
\begin{subfigure}[b]{0.33\textwidth}
  \pgfplotsset{corranal/.style={
      width=60mm,
      height=30mm,
      xmin=0,
      xmax=1,
      ymin=0,
      ymax=1.1,
      %xtick={1, 2, 3, 4, 5, 6},
      %xticklabels={1\%, 2\%, 4\%, 8\%, 16\%, 32\%},
      ytick={0, 0.2, ..., 1.0},
      %bar width=7pt,
      ylabel near ticks,
      ylabel shift=-2pt,
      xlabel near ticks,
      ylabel style={align=center},
      %xmode=log,
      xlabel=True Correlation Parameter,
      ylabel=Learned\\ Corr Param,
      legend style={
        at={(0.37,1)},anchor=south west,column sep=3pt,
        draw=none,font=\scriptsize,fill=none,font=\scriptsize,line width=.5pt,
        /tikz/every even column/.append style={column sep=5pt}
      },
      legend columns=3,
      every axis/.append style={font=\scriptsize},
      %area legend,
      tick style={draw=none},
      legend cell align=left,
      xmajorgrids,
      ymajorgrids,
      %legend image post style={darkorange,line width=1pt},
  }}

  \pgfplotsset{scatterdots/.style={
      fill=gray,
      draw=none,
      only marks,
      mark size=1.5,
      opacity=0.8,
  }}

  \centering
  \begin{tikzpicture}
    \begin{axis}[corranal]

      \addplot[scatterdots]
      table[x=x,y=y1] {data/cov_analysis.csv};

      \addplot[scatterdots,fill=darkteal]
      table[x=x,y=y2] {data/cov_analysis.csv};

      \addplot[scatterdots,fill=darkorange]
      table[x=x,y=y3] {data/cov_analysis.csv};

      \addplot[draw=black,mark=none] coordinates {(0,0) (1,1)};

      %\addplot[scatterdots,fill=red,draw=black!50!red]
      %table[x=x,y=y4] {data/cov_analysis.csv};

      \addlegendentry{20};
      \addlegendentry{50};
      \addlegendentry{100};
    \end{axis}

    \node[font=\scriptsize] at (0.7,1.7) {\# past queries:};

  \end{tikzpicture}
  %\vspace{-3mm}

  \caption{Correlation Param Learning}
\end{subfigure}
~
\begin{subfigure}[b]{0.33\textwidth}
  \pgfplotsset{confsize/.style={
      width=60mm,
      height=30mm,
      xmin=0,
      xmax=1,
      ymin=0,
      ymax=0.2,
      xtick={0, 0.2, ..., 1},
      ytick={0, 0.05, 0.1, 0.15, 0.2},
      yticklabels={0, 5, 10, 15, 20},
      %bar width=7pt,
      ylabel near ticks,
      ylabel shift=-2pt,
      xlabel near ticks,
      ylabel style={align=center},
      %xmode=log,
      xlabel=Correlation Parameter,
      ylabel=Actual Error Ratio\\ to Guaranteed\\ Errors (\%),
      legend style={
        at={(-0.1,1)},anchor=south west,column sep=3pt,
        draw=none,font=\scriptsize,fill=none,line width=.5pt},
      legend columns=2,
      every axis/.append style={font=\scriptsize},
      %area legend,
      tick style={draw=none},
      ymajorgrids,
      legend cell align=left
      %legend image post style={darkorange,line width=1pt},
  }}

  \pgfplotsset{graybar/.style={
      fill=none,
      draw=darkteal,
      ultra thick,
  }}


  \centering
  \begin{tikzpicture}
    \begin{axis}[confsize]

      \addplot[graybar,
          error bars/.cd,
          y dir=both,
          y explicit,
          error bar style={line width=0.5pt,darkorange},
          error mark options={
              rotate=90,
              darkorange,
              mark size=2pt,
              line width=1pt
          },
      ]
      coordinates {
        (0.050, 0.09) +- (0.25, 0.08)
        (0.100, 0.09) +- (0.19, 0.08)
        (0.150, 0.07) +- (0.19, 0.06)
        (0.200, 0.09) +- (0.17, 0.08)
        (0.250, 0.08) +- (0.18, 0.07)
        (0.300, 0.06) +- (0.11, 0.06)
        (0.350, 0.05) +- (0.11, 0.04)
        (0.400, 0.04) +- (0.1, 0.03 )
        (0.450, 0.05) +- (0.11, 0.04)
        (0.500, 0.04) +- (0.11, 0.04)
        (0.550, 0.04) +- (0.07, 0.04)
        (0.600, 0.03) +- (0.05, 0.03)
        (0.650, 0.03) +- (0.07, 0.03)
        (0.700, 0.03) +- (0.06, 0.03)
        (0.750, 0.03) +- (0.06, 0.03)
        (0.800, 0.03) +- (0.05, 0.03)
        (0.850, 0.04) +- (0.1, 0.04 )
        (0.900, 0.04) +- (0.06, 0.04)
        (0.950, 0.03) +- (0.07, 0.03)
      };

      \addplot[draw=darkorange,ultra thick] coordinates {(8,0)};

      \addlegendentry{median};
      \addlegendentry{5\%, 95\% percentiles};
    \end{axis}


  \end{tikzpicture}
  %\vspace{-3mm}

  \caption{Validity of ME Principle}
\end{subfigure}
~
%\begin{subfigure}[b]{0.24\textwidth}
%  \pgfplotsset{paramest/.style={
%      width=45mm,
%      height=28mm,
%      xtick={1, 2, 3, 4, 5, 6, 7, 8},
%      xticklabels={-10\%, -5\%, -2\%, -1\%, 1\%, 2\%, 5\%, 10\%},
%      ytick={0,5,10,15,20},
%      xmin=0.5,
%      xmax=8.5,
%      ymin=0,
%      ymax=20,
%      bar width=3pt,
%      %xmode=log,
%      xlabel near ticks,
%      xlabel shift=-8pt,
%      ylabel shift=-3pt,
%      xlabel near ticks,
%      xlabel style={align=center},
%      xlabel=Relative Parameter Error (\%),
%      ylabel=Conf Interval\\ Violation (\%),
%      ylabel style={align=center},
%      legend style={
%        at={(0,1)},anchor=south west,column sep=2pt,
%        draw=none,font=\scriptsize,fill=none,line width=.5pt,
%        /tikz/every even column/.append style={column sep=7pt}
%      },
%      legend columns=2,
%      every axis/.append style={font=\scriptsize},
%      ybar=1.5pt,
%      area legend,
%      xtick style={draw=none},
%      ymajorgrids,
%      legend cell align=left,
%      x tick label style={rotate=60, anchor=east,xshift=3pt},
%      %nodes near coords
%  }}
%
%  \pgfplotsset{tealbar/.style={
%      draw=black!50!darkteal,
%      fill=darkteal,
%  }}
%
%  \pgfplotsset{redbar/.style={
%      draw=black!50!darkorange,
%      fill=darkorange,
%  }}
%
%  \centering
%  \begin{tikzpicture}
%    \begin{axis}[paramest]
%
%      \addplot[tealbar]   % stat error
%      table[x=x,y=y]{
%        x	y
%        1	10.5
%        2	12.6
%        3	13.7
%        4	8.7
%        5	8.7
%        6	15.5
%        7	8.9
%        8	10.8
%      };
%
%      \addplot[redbar]   % actual error
%      table[x=x,y=y]{
%        x	y
%        1	1.2
%        2	1.0
%        3	0.8
%        4	0.3
%        5	0.0
%        6	0.2
%        7	1.5
%        8	0.2
%      };
%
%      \addlegendentry{w/o guard};
%      \addlegendentry{w/ guard};
%
%    \end{axis}
%  \end{tikzpicture}
%  \caption{Under/Over Estimation}
%\end{subfigure}
%~
\begin{subfigure}[b]{0.33\textwidth}
  \pgfplotsset{confsize/.style={
      width=60mm,
      height=30mm,
      xmin=0,
      xmax=1,
      ymin=0.6,
      ymax=2.2,
      xtick={0, 0.2, ..., 1},
      ytick={0.6, 1.0, ..., 2.2},
      %bar width=7pt,
      ylabel near ticks,
      ylabel shift=-2pt,
      xlabel near ticks,
      ylabel style={align=center},
      %xmode=log,
      xlabel=Correlation Parameter,
      ylabel=\dbl Error Bound\\ to True Error Bound,
      legend style={
        at={(-0.1,1)},anchor=south west,column sep=3pt,
        draw=none,font=\scriptsize,fill=none,line width=.5pt},
      legend columns=2,
      every axis/.append style={font=\scriptsize},
      %area legend,
      tick style={draw=none},
      ymajorgrids,
      legend cell align=left
      %legend image post style={darkorange,line width=1pt},
  }}

  \pgfplotsset{graybar/.style={
      fill=none,
      draw=darkteal,
      ultra thick,
  }}

  \centering
  \begin{tikzpicture}
    \begin{axis}[
        confsize,
      ]

      \addplot[graybar,
          error bars/.cd,
          y dir=both,
          y explicit,
          error bar style={line width=0.5pt,darkorange},
          error mark options={
              rotate=90,
              darkorange,
              mark size=2pt,
              line width=1pt
          },
      ]
      %]   % baseline
      %plot[error bars/.cd, y dir=both,y explicit,line width=2pt]
      coordinates {
        (0.050, 1.000) +- (0.003, 0.021)
      (0.100, 1.000) +- (0.031, 0.000)
      (0.150, 1.004) +- (0.073, 0.019)
      (0.200, 1.005) +- (0.295, 0.051)
      (0.250, 1.000) +- (0.010, 0.117)
      (0.300, 1.005) +- (0.194, 0.126)
      (0.350, 1.019) +- (0.382, 0.132)
      (0.400, 1.000) +- (1.084, 0.133)
      (0.450, 1.051) +- (0.279, 0.051)
      (0.500, 1.132) +- (0.357, 0.132)
      (0.550, 1.028) +- (0.032, 0.028)
      (0.600, 1.052) +- (0.074, 0.052)
      (0.650, 1.376) +- (0.693, 0.543)
      (0.700, 1.132) +- (0.110, 0.132)
      (0.750, 1.154) +- (0.132, 0.154)
      (0.800, 1.143) +- (0.115, 0.143)
      (0.850, 1.078) +- (0.054, 0.047)
      (0.900, 1.052) +- (0.039, 0.033)
      (0.950, 1.053) +- (0.055, 0.053)
      };

      \addplot[draw=darkorange,ultra thick] coordinates {(8,0)};

      \addlegendentry{median};
      \addlegendentry{5\%, 95\% percentiles};

    \end{axis}
  \end{tikzpicture}

  \caption{\dbl's Confidence Interval Size}
\end{subfigure}

\caption{\tofix{\dbl's correlation learning and the conditions for its
correctness:
(a) \dbl's correlation learning accuracy,
(b) the validity of the maximum entropy principle (assumption for
Theorem~\ref{thm:accuracy}).
(c) the condition for the correctness of \dbl's error bounds
(in Theorem~\ref{thm:accuracy}),
In (b), the validity is satisfied if the ratio is equal to or smaller than 100\%.
In (c), the condition is satisfied when the ratio is equal to or larger than 1.0.
}}
\label{fig:exp:correlation}
%\vspace{\neggap}
\end{figure*}




==> fig_exp_correlation_new.tex <==
\begin{figure*}[t]
  \hspace*{-2mm}
\begin{subfigure}[b]{0.33\textwidth}
  \pgfplotsset{corranal/.style={
      width=60mm,
      height=30mm,
      xmin=0,
      xmax=1,
      ymin=0,
      ymax=1.1,
      %xtick={1, 2, 3, 4, 5, 6},
      %xticklabels={1\%, 2\%, 4\%, 8\%, 16\%, 32\%},
      ytick={0, 0.2, ..., 1.0},
      %bar width=7pt,
      ylabel near ticks,
      ylabel shift=-2pt,
      xlabel near ticks,
      ylabel style={align=center},
      %xmode=log,
      xlabel=True Correlation Parameter,
      ylabel=Learned\\ Corr Param,
      legend style={
        at={(0.37,1)},anchor=south west,column sep=3pt,
        draw=none,font=\scriptsize,fill=none,font=\scriptsize,line width=.5pt,
        /tikz/every even column/.append style={column sep=5pt}
      },
      legend columns=3,
      every axis/.append style={font=\scriptsize},
      %area legend,
      tick style={draw=none},
      legend cell align=left,
      xmajorgrids,
      ymajorgrids,
      %legend image post style={darkorange,line width=1pt},
  }}

  \pgfplotsset{scatterdots/.style={
      fill=gray,
      draw=none,
      only marks,
      mark size=1.5,
      opacity=0.8,
  }}

  \centering
  \begin{tikzpicture}
    \begin{axis}[corranal]

      \addplot[scatterdots]
      table[x=x,y=y1] {data/cov_analysis.csv};

      \addplot[scatterdots,fill=darkteal]
      table[x=x,y=y2] {data/cov_analysis.csv};

      \addplot[scatterdots,fill=darkorange]
      table[x=x,y=y3] {data/cov_analysis.csv};

      \addplot[draw=black,mark=none] coordinates {(0,0) (1,1)};

      %\addplot[scatterdots,fill=red,draw=black!50!red]
      %table[x=x,y=y4] {data/cov_analysis.csv};

      \addlegendentry{20};
      \addlegendentry{50};
      \addlegendentry{100};
    \end{axis}

    \node[font=\scriptsize] at (0.7,1.7) {\# past queries:};

  \end{tikzpicture}
  %\vspace{-3mm}

  \caption{Correlation Param Learning}
\end{subfigure}
~
\begin{subfigure}[b]{0.33\textwidth}
  \pgfplotsset{confsize/.style={
      width=60mm,
      height=30mm,
      xmin=0.5,
      xmax=7.5,
      ymin=0,
      ymax=4.2,
      ybar,
      bar width=5pt,
      xtick={1, 2, ..., 7},
      xticklabels={0.1, 0.2, 0.5, 1.0, 2.0, 5.0, 10.0},
      ytick={0, 1, 2, 3, 4},
      %yticklabels={0, 100, 200, 300, 400},
      %bar width=7pt,
      ylabel near ticks,
      ylabel shift=-2pt,
      %xlabel shift=-2pt,
      %xlabel near ticks,
      ylabel style={align=center},
      %xmode=log,
      xlabel=Artificial Correlation Parameter Scale (x),
      ylabel=Ratio of\\ Actual Error to \\ Guaranteed Error,
      legend style={
        at={(0.02,1.3)},anchor=north west,column sep=3pt,
        draw=black,font=\tiny,fill=white,line width=.5pt,
        %/tikz/every even column/.append style={column sep=15pt}
      },
      legend columns=1,
      every axis/.append style={font=\scriptsize},
      %area legend,
      tick style={draw=none},
      ymajorgrids,
      legend cell align=left,
      x tick label style={yshift=2pt},
      %legend image post style={darkorange,line width=1pt},
  }}

  \pgfplotsset{graybar/.style={
      fill=none,
      draw=none,
      error bars/.cd,
      y dir=both,
      y explicit,
      error bar style={line width=0.5pt,black},
      error mark options={
          rotate=90,
          darkteal,
          mark size=3pt,
          line width=1.5pt
      },
  }}

  \pgfplotsset{redbar/.style={
      fill=none,
      draw=none,
      error bars/.cd,
      y dir=both,
      y explicit,
      error bar style={line width=0.5pt,black!50!darkorange},
      error mark options={
          rotate=90,
          darkorange,
          mark size=3pt,
          line width=1.5pt
      },
  }}

  \tikzset{mediandot/.style={
    scale=0.5,fill=darkteal,draw=black!50!darkteal,rectangle,
  }}

  \pgfplotsset{
    box legend image/.style={
      legend image code/.code={%
        \node[minimum width=1.5mm,minimum height=1mm,
              fill=#1,draw=black!50!#1,inner sep=0]
        at (0.2cm,0cm) {};
      }
    },
  }

  \pgfplotsset{
    errorbar legend image/.style={
      legend image code/.code={%
        \draw[ultra thick,#1] (0.1cm,0cm)--(0.4cm,0cm);
      }
    },
  }


  \centering
  \begin{tikzpicture}
    \begin{axis}[confsize]
      \addlegendimage{box legend image=darkteal};
      \addlegendentry{Median w/o safeguard};

      \addlegendimage{errorbar legend image=darkteal};
      \addlegendentry{5\%, 95\% pctl w/o safeguard};

      \addlegendimage{box legend image=darkorange};
      \addlegendentry{Median w/ safeguard};

      \addlegendimage{errorbar legend image=darkorange};
      \addlegendentry{5\%, 95\% pctl w/ safeguard};


      \addplot[graybar]
      table [y error plus=z2, y error minus=z1] {
        x	y	z1	z2
        1	0.09	0.08	0.22
        2	0.09	0.08	0.22
        3	0.08	0.08	0.15
        4	0.09	0.08	0.20
        5	0.24	0.22	0.57
        6	0.68	0.64	2.32
        7	1.13	1.04	2.96
      };

      \addplot[redbar]
      table [y error plus=z2, y error minus=z1] {
        x	y	z1	z2
        1	0.08	0.07	0.23
        2	0.08	0.08	0.17
        3	0.07	0.06	0.16
        4	0.08	0.07	0.22
        5	0.15	0.14	0.26
        6	0.13	0.11	0.56
        7	0.11	0.10	0.49
      };

      \node[mediandot] at (axis cs:0.8, 0.09) {};
      \node[mediandot] at (axis cs:1.8, 0.09) {};
      \node[mediandot] at (axis cs:2.8, 0.08) {};
      \node[mediandot] at (axis cs:3.8, 0.09) {};
      \node[mediandot] at (axis cs:4.8, 0.24) {};
      \node[mediandot] at (axis cs:5.8, 0.68) {};
      \node[mediandot] at (axis cs:6.8, 1.13) {};

      \node[mediandot,fill=darkorange,draw=black!50!darkorange] at (axis cs:1.2, 0.08) {};
      \node[mediandot,fill=darkorange,draw=black!50!darkorange] at (axis cs:2.2, 0.08) {};
      \node[mediandot,fill=darkorange,draw=black!50!darkorange] at (axis cs:3.2, 0.07) {};
      \node[mediandot,fill=darkorange,draw=black!50!darkorange] at (axis cs:4.2, 0.08) {};
      \node[mediandot,fill=darkorange,draw=black!50!darkorange] at (axis cs:5.2, 0.15) {};
      \node[mediandot,fill=darkorange,draw=black!50!darkorange] at (axis cs:6.2, 0.13) {};
      \node[mediandot,fill=darkorange,draw=black!50!darkorange] at (axis cs:7.2, 0.11) {};


      %\addplot[draw=darkorange,ultra thick] coordinates {(8,0)};

    \end{axis}


  \end{tikzpicture}
  %\vspace{-3mm}

  \caption{Validity of ME Principle / Effect of Safeguard}
\end{subfigure}
~
%\begin{subfigure}[b]{0.24\textwidth}
%  \pgfplotsset{paramest/.style={
%      width=45mm,
%      height=28mm,
%      xtick={1, 2, 3, 4, 5, 6, 7, 8},
%      xticklabels={-10\%, -5\%, -2\%, -1\%, 1\%, 2\%, 5\%, 10\%},
%      ytick={0,5,10,15,20},
%      xmin=0.5,
%      xmax=8.5,
%      ymin=0,
%      ymax=20,
%      bar width=3pt,
%      %xmode=log,
%      xlabel near ticks,
%      xlabel shift=-8pt,
%      ylabel shift=-3pt,
%      xlabel near ticks,
%      xlabel style={align=center},
%      xlabel=Relative Parameter Error (\%),
%      ylabel=Conf Interval\\ Violation (\%),
%      ylabel style={align=center},
%      legend style={
%        at={(0,1)},anchor=south west,column sep=2pt,
%        draw=none,font=\scriptsize,fill=none,line width=.5pt,
%        /tikz/every even column/.append style={column sep=7pt}
%      },
%      legend columns=2,
%      every axis/.append style={font=\scriptsize},
%      ybar=1.5pt,
%      area legend,
%      xtick style={draw=none},
%      ymajorgrids,
%      legend cell align=left,
%      x tick label style={rotate=60, anchor=east,xshift=3pt},
%      %nodes near coords
%  }}
%
%  \pgfplotsset{tealbar/.style={
%      draw=black!50!darkteal,
%      fill=darkteal,
%  }}
%
%  \pgfplotsset{redbar/.style={
%      draw=black!50!darkorange,
%      fill=darkorange,
%  }}
%
%  \centering
%  \begin{tikzpicture}
%    \begin{axis}[paramest]
%
%      \addplot[tealbar]   % stat error
%      table[x=x,y=y]{
%        x	y
%        1	10.5
%        2	12.6
%        3	13.7
%        4	8.7
%        5	8.7
%        6	15.5
%        7	8.9
%        8	10.8
%      };
%
%      \addplot[redbar]   % actual error
%      table[x=x,y=y]{
%        x	y
%        1	1.2
%        2	1.0
%        3	0.8
%        4	0.3
%        5	0.0
%        6	0.2
%        7	1.5
%        8	0.2
%      };
%
%      \addlegendentry{w/o guard};
%      \addlegendentry{w/ guard};
%
%    \end{axis}
%  \end{tikzpicture}
%  \caption{Under/Over Estimation}
%\end{subfigure}
%~
\begin{subfigure}[b]{0.33\textwidth}
  \pgfplotsset{confsize/.style={
      width=60mm,
      height=30mm,
      xmin=0,
      xmax=1,
      ymin=0.9,
      ymax=1.3,
      xtick={0, 0.2, ..., 1},
      ytick={0.9, 1.0, ..., 1.4},
      %bar width=7pt,
      ylabel near ticks,
      ylabel shift=-2pt,
      xlabel shift=-2pt,
      xlabel near ticks,
      ylabel style={align=center},
      %xmode=log,
      xlabel=True Correlation Parameter,
      ylabel=Ratio of\\ \dbl Error Bound\\ to True Error Bound,
      legend style={
        at={(-0.1,1)},anchor=south west,column sep=3pt,
        draw=none,font=\scriptsize,fill=none,line width=.5pt},
      legend columns=2,
      every axis/.append style={font=\scriptsize},
      %area legend,
      tick style={draw=none},
      ymajorgrids,
      legend cell align=left
      %legend image post style={darkorange,line width=1pt},
  }}

  \pgfplotsset{graybar/.style={
      fill=none,
      draw=darkteal,
      ultra thick,
  }}

  \centering
  \begin{tikzpicture}
    \begin{axis}[
        confsize,
      ]

      \addplot[graybar,
          error bars/.cd,
          y dir=both,
          y explicit,
          error bar style={line width=0.5pt,darkorange},
          error mark options={
              rotate=90,
              darkorange,
              mark size=2pt,
              line width=1pt
          },
      ]
      table [y error plus=z2, y error minus=z1] {
        x	y	z1	z2
        0.050	1.003	0.025	0.032
        0.100	1.000	0.002	0.003
        0.150	1.024	0.040	0.021
        0.200	1.028	0.042	0.025
        0.250	1.013	0.023	0.011
        0.300	1.003	0.013	0.006
        0.350	1.025	0.019	0.020
        0.400	1.081	0.073	0.055
        0.450	1.016	0.017	0.012
        0.500	1.074	0.058	0.051
        0.550	1.046	0.032	0.031
        0.600	1.057	0.036	0.044
        0.650	1.181	0.110	0.106
        0.700	1.067	0.033	0.043
        0.750	1.083	0.043	0.051
        0.800	1.084	0.060	0.058
        0.850	1.058	0.031	0.029
        0.900	1.039	0.026	0.021
        0.950	1.039	0.029	0.024
      };

      \addplot[draw=darkorange,ultra thick] coordinates {(8,0)};

      \addlegendentry{Median};
      \addlegendentry{5\%, 95\% percentiles};

    \end{axis}
  \end{tikzpicture}

  \caption{\dbl's Error Bound Size compared to True}
\end{subfigure}

\caption{\rev{
(a) The accuracy of \dbl's correlation parameter learning,
(b) the validity of the ME principle (Theorem~\ref{thm:accuracy}'s assumption) and the effectiveness of our safeguard, and
(c) the ratio of \dbl's error bounds to true error bounds
(Theorem~\ref{thm:accuracy}'s condition).
In (b), 95\% percentiles being lower than 1 indicates their probabilistic
correctness.
In (c), the condition in Theorem~\ref{thm:accuracy} is satisfied if the ratio is equal to or larger than 1.
}}
\label{fig:exp:correlation}
%\vspace{\neggap}
\end{figure*}




==> fig_exp_error_red.tex <==
% 1. Overall speedup for cached (both TPCH and Vertica)
% 2. Overall speedup for non-cached (both TPCH and Vertica)
% 3. Average-latency graph for cached (Vertica)
% 4. Average-latency graph for non-cached (Vertica)
% May non include this: 5. Average-latency graph for cached (TPCH)
% May non include this: 6. Average-latency graph for non-cached (TPCH)

\begin{figure}

  \pgfplotsset{speedupgraph/.style={
      width=40mm,
      height=30mm,
      xtick={1, 2},
      xticklabels={\vertica, \tpch},
      %ytick={0,20,40,60},
      xmin=0.5,
      xmax=2.5,
      ymin=0,
      ymax=120,
      ytick={0, 20, ..., 100},
      bar width=7pt,
      %xmode=log,
      xlabel near ticks,
      xlabel shift=-2pt,
      ylabel shift=-2pt,
      xlabel near ticks,
      xlabel style={align=center},
      ylabel style={align=center},
      ylabel=Error\\ Reduction (\%),
      legend style={
        at={(0,1.1)},anchor=south west,column sep=2pt,
        draw=none,font=\scriptsize,fill=none,line width=.5pt,
        /tikz/every even column/.append style={column sep=20pt}
      },
      legend columns=2,
      every axis/.append style={font=\scriptsize},
      ybar=5pt,
      area legend,
      xtick style={draw=none},
      nodes near coords
  }}

  \pgfplotsset{graybar/.style={
      draw=black!50!darkteal,
      fill=darkteal,
  }}

  \pgfplotsset{redbar/.style={
      draw=black!50!darkorange,
      fill=darkorange,
  }}

  \begin{subfigure}[b]{0.45\linewidth}
    \centering
    \begin{tikzpicture}
      \begin{axis}[
          speedupgraph,
        ]

        \addplot[graybar]
        table[x=x,y=y]{
          x	y
          1	88.89
          2	55.92
        };

      %\addlegendentry{\nol};
      %\addlegendentry{\dbl};
      \end{axis}
    \end{tikzpicture}

    \caption{Cached}
  \end{subfigure}
  ~
  \begin{subfigure}[b]{0.48\linewidth}
    \centering
    \begin{tikzpicture}
      \begin{axis}[
          speedupgraph,
        ]

        \addplot[graybar]   % baseline
        table[x=x,y=y]{
          x	y
          1	92.58
          2	95.33
        };

      \end{axis}
    \end{tikzpicture}

    \caption{Not Cached}
  \end{subfigure}

  \caption{Average error reduction of queries by \dbl (compared to \nol) for the same time budget.}
  \label{fig:exp:error_red}
  \vspace{\neggap}
\end{figure}


==> fig_exp_overhead.tex <==
\begin{figure}

  \pgfplotsset{overhead/.style={
      width=60mm,
      height=30mm,
      %ytick={0, 1, 2, 3, 4},
      %ytick={0,20,40,60},
      xtick={1, 2},
      xticklabels={Cached, No-Cache},
      xmin=0.5,
      xmax=2.5,
      ymin=0,
      ymax=60,
      bar width=14pt,
      %xmode=log,
      ylabel style={align=center},
      ylabel=Latency (sec),
      legend style={at={(0,1)},anchor=north west,column sep=2pt,
        draw=none,font=\scriptsize},
      legend columns=1,
      every axis/.append style={font=\scriptsize},
      ybar stacked,
      area legend,
      legend cell align=left,
      xtick style={draw=none},
  }}

  \pgfplotsset{graybar/.style={
      fill=darkteal,
      draw=none,
  }}
  \pgfplotsset{redbar/.style={
      draw=none,
      fill=darkorange,
  }}

  \centering
  \begin{tikzpicture}
    \begin{axis}[
        overhead,
      ]

      \addplot[graybar]   % baseline
      table[x=x,y=y]{
        x	y
        1	2.083
        2	52.5
      };

      \addplot[redbar]   % overhead
      table[x=x,y=y]{
        x	y
        1	0.02
        2	0.5
      };
     % real value: 9.95
     % real value: 10.24

      \addlegendentry{Basic};
      \addlegendentry{Overhead};

    \end{axis}
  \end{tikzpicture}

  \caption{Overhead of \dbl compared to regular query processing. The overheads
    for both cases were too small to be easily noticeable. On
    average, \dbl's overhead were 0.52\% for querying data cached in memory and 0.12\% for
  querying data stored in SSD devices.}
  \label{fig:exp:overhead}
  \vspace{\neggap}
\end{figure}




==> fig_exp_set.tex <==
\begin{figure*}[t]
\centering

  \pgfplotsset{statcorrect/.style={
      width=70mm,
      height=30mm,
      xmin=0.5,
      xmax=6.5,
      ymin=0,
      ymax=25,
      xtick={1, 2, 3, 4, 5, 6},
      xticklabels={1\%, 2\%, 4\%, 8\%, 16\%, 32\%},
      ytick={0, 5, ..., 25},
      %bar width=7pt,
      ylabel near ticks,
      ylabel shift=-2pt,
      xlabel near ticks,
      ylabel style={align=center},
      %xmode=log,
      xlabel=Guaranteed Error (\%),
      ylabel=Actual Error (\%),
      legend style={
        at={(0,1)},anchor=north west,column sep=3pt,
        draw=none,font=\scriptsize,fill=none,font=\tiny,line width=.5pt},
      legend columns=1,
      every axis/.append style={font=\scriptsize},
      %area legend,
      tick style={draw=none},
      ymajorgrids,
      legend cell align=left
      %legend image post style={darkorange,line width=1pt},
  }}

  \pgfplotsset{contgraph/.style={
      width=40mm,
      height=30mm,
      xtick={1, 2},
      xticklabels={stat err, actual err},
      ytick={0,0.2,...,1.0},
      yticklabels={0,20,40,60,80,100},
      xmin=0.5,
      xmax=2.5,
      ymin=0,
      ymax=1.1,
      bar width=7pt,
      %xmode=log,
      xlabel near ticks,
      xlabel shift=-2pt,
      ylabel shift=-2pt,
      xlabel near ticks,
      xlabel style={align=center},
      ylabel=Speedup (x),
      legend style={
        at={(0,1.1)},anchor=south west,column sep=2pt,
        draw=none,font=\scriptsize,fill=none,line width=.5pt,
        /tikz/every even column/.append style={column sep=20pt}
      },
      legend columns=2,
      every axis/.append style={font=\scriptsize},
      ybar=5pt,
      area legend,
      xtick style={draw=none},
      nodes near coords
  }}

  \pgfplotsset{tealbar/.style={
      draw=black!50!darkteal,
      fill=darkteal,
  }}

  \pgfplotsset{graybar/.style={
      fill=none,
      draw=darkteal,
      ultra thick,
  }}

\begin{subfigure}[b]{0.25\textwidth}
  \centering
  \begin{tikzpicture}
    \begin{axis}[contgraph]

      \addplot[tealbar]   % intelli
      table[x=x,y=y]{
        x	y
        1	0.8109147515
        2	0.7908743991
      };

      \addplot[tealbar]   % SmartCache
      table[x=x,y=y]{
        x	y
        1	0.5991453754
        2	0.5925314709
      };
    \end{axis}
  \end{tikzpicture}

  \caption{}
\end{subfigure}
~
\begin{subfigure}[b]{0.40\textwidth}
  \centering
  \begin{tikzpicture}
    \begin{axis}[statcorrect]

      \addplot[graybar,
        error bars/.cd,
        y dir=both,
        y explicit,
        error bar style={line width=0.5pt,darkorange},
        error mark options={
            rotate=90,
            darkorange,
            mark size=4pt,
            line width=1pt
        },
      ]
      %]   % baseline
      %plot[error bars/.cd, y dir=both,y explicit,line width=2pt]
      coordinates {
        (1, 0.099) +-  (0.253, 0.095)
        (2, 0.899) +-  (2.264, 0.874)
        (3, 1.054) +-  (1.376, 0.878)
        (4, 3.490) +-  (5.338, 3.176)
        (5, 6.027) +- (8.906, 5.506)
        (6, 11.144) +-(8.008, 10.372)
      };

      \addplot[draw=darkorange,ultra thick] coordinates {(8,0)};

      \addlegendentry{mean};
      \addlegendentry{5\%, 95\% percentiles};

    \end{axis}
  \end{tikzpicture}
  \caption{}
\end{subfigure}
~
\begin{subfigure}[b]{0.32\textwidth}
  \centering
  \small

  \vspace{2mm}

  \begin{tabular}{|l|r|r|}
    \hline
    \textbf{Latency }    & \textbf{Cached} & \textbf{No-Cache} \\ \Xhline{2\arrayrulewidth}
    \nol                 & 2.083 sec       & 52.50 sec \\ \hline
    \dbl                 & 2.093 sec       & 52.51 sec \\ \hline
    \textbf{Overhead}    & 0.010 sec       & 0.010 sec \\ \hline
  \end{tabular}
  \caption{}
\end{subfigure}

\caption{(a) \tofix{contribution of correlation modeling}
(b) correctness of \dbl's statistical error guarantees, (c) The runtime overhead of \dbl.}
  \label{fig:exp:staterror}
\label{tab:exp:overhead}

\vspace{\neggap}
\end{figure*}




==> fig_exp_speedup.tex <==
% 1. Overall speedup for cached (both TPCH and Vertica)
% 2. Overall speedup for non-cached (both TPCH and Vertica)
% 3. Average-latency graph for cached (Vertica)
% 4. Average-latency graph for non-cached (Vertica)
% May non include this: 5. Average-latency graph for cached (TPCH)
% May non include this: 6. Average-latency graph for non-cached (TPCH)

\begin{figure*}
  \pgfplotsset{speedupgraph/.style={
      width=45mm,
      height=35mm,
      xtick={1, 2},
      xticklabels={\vertica, \tpch},
      %ytick={0,20,40,60},
      xmin=0.5,
      xmax=2.5,
      ymin=0,
      bar width=7pt,
      %xmode=log,
      xlabel near ticks,
      xlabel shift=-2pt,
      ylabel shift=-2pt,
      xlabel near ticks,
      xlabel style={align=center},
      ylabel=Speedup (x),
      legend style={
        at={(0,1.1)},anchor=south west,column sep=2pt,
        draw=none,font=\scriptsize,fill=none,line width=.5pt,
        /tikz/every even column/.append style={column sep=20pt}
      },
      legend columns=2,
      every axis/.append style={font=\scriptsize},
      ybar=10pt,
      area legend,
      xtick style={draw=none},
      x tick label style={yshift=5pt},
      nodes near coords
  }}

  \pgfplotsset{errredgraph/.style={
      width=45mm,
      height=35mm,
      xtick={1, 2},
      xticklabels={\vertica, \tpch},
      %ytick={0,20,40,60},
      xmin=0.5,
      xmax=2.5,
      ymin=0,
      ymax=120,
      ytick={0, 20, ..., 100},
      bar width=7pt,
      %xmode=log,
      xlabel near ticks,
      xlabel shift=-2pt,
      ylabel shift=-2pt,
      xlabel near ticks,
      xlabel style={align=center},
      ylabel style={align=center},
      ylabel=Error\\ Reduction (\%),
      legend style={
        at={(0,1.1)},anchor=south west,column sep=2pt,
        draw=none,font=\scriptsize,fill=none,line width=.5pt,
        /tikz/every even column/.append style={column sep=20pt}
      },
      legend columns=2,
      every axis/.append style={font=\scriptsize},
      ybar=10pt,
      area legend,
      xtick style={draw=none},
      x tick label style={yshift=5pt},
      nodes near coords
  }}

  \pgfplotsset{redbar/.style={
      draw=black!50!darkteal,
      fill=darkteal,
  }}

  \pgfplotsset{graybar/.style={
      draw=black!50!darkorange,
      fill=darkorange,
      postaction={
        pattern=north west lines,
      }
  }}

  \begin{subfigure}[b]{0.23\textwidth}
    \centering
    \begin{tikzpicture}
      \begin{axis}[
          speedupgraph,
          ymin=0,
          ymax=3.5,
          ytick={0, 1, ..., 4},
        ]

        \addplot[graybar]   % speedup
        table[x=x,y=y]{
          x	y
          1	2.01
          2	2.63
        };

        \addplot[redbar]   % speedup
        table[x=x,y=y]{
          x	y
          1	1.58
          2	1.87
        };

        %\addplot[graybar]   % baseline
        %table[x=x,y=y]{
        %  x	y
        %  1	3.38
        %  2	1.07
        %};

        %\addplot[redbar]
        %table[x=x,y=y]{
        %  x	y
        %  1	1.68
        %  2	0.405
        %};

        \addlegendentry{Speedup and Error reduction based on estimated errors};

      %\addlegendentry{\nol};
      %\addlegendentry{\dbl};
      \end{axis}
    \end{tikzpicture}

    \caption{Cached}
  \end{subfigure}
  ~
  \begin{subfigure}[b]{0.23\textwidth}
    \centering
    \begin{tikzpicture}
      \begin{axis}[
          speedupgraph,
          ymin=0,
          ymax=16,
          ytick={0, 4, 8, 12, 16},
        ]

        \addplot[graybar]   % baseline
        table[x=x,y=y]{
          x	y
          1	10.43
          2	4.09
        };

        \addplot[redbar]   % speedup
        table[x=x,y=y]{
          x	y
          1	13.61
          2	4.07
        };

        %\addplot[graybar]   % baseline
        %table[x=x,y=y]{
        %  x	y
        %  1	167
        %  2	34.3
        %};

        %\addplot[redbar]
        %table[x=x,y=y]{
        %  x	y
        %  1	16
        %  2	8.4
        %};

      \end{axis}
    \end{tikzpicture}

    \caption{Not Cached}
  \end{subfigure}
  ~
  \begin{subfigure}[b]{0.24\textwidth}
    \centering
    \begin{tikzpicture}
      \begin{axis}[
          errredgraph,
        ]

        \addplot[graybar]
        table[x=x,y=y]{
          x	y
          1	88.89
          2	55.92
        };

        \addplot[redbar]
        table[x=x,y=y]{
          x	y
          1	89.10
          2	45.18
        };

        \legend{,Speedup and Error reduction based on actual errors};

      %\addlegendentry{\nol};
      %\addlegendentry{\dbl};
      \end{axis}
    \end{tikzpicture}

    \caption{Cached}
  \end{subfigure}
  ~
  \begin{subfigure}[b]{0.24\textwidth}
    \centering
    \begin{tikzpicture}
      \begin{axis}[
          errredgraph,
        ]

        \addplot[graybar]   % stat error
        table[x=x,y=y]{
          x	y
          1	92.58
          2	95.33
        };

        \addplot[redbar]   % actual error
        table[x=x,y=y]{
          x	y
          1	90.71
          2	88.45
        };

      \end{axis}
    \end{tikzpicture}

    \caption{Not Cached}
  \end{subfigure}

  \caption{
    \rev{Speedup of \dbl over \nol for a target error of 2\% (a-b) and average error reduction of queries by \dbl
  (compared to \nol) for the same time budget (c-d).
  %In practice, users are provided only estimated errors.
  }
  % This figure's speedups were based on 0.5\% statistical error
    % for the \vertica dataset and 2\% for the \tpch dataset.
    }
  \label{fig:exp:speedup}
\end{figure*}


==> fig_exp_stat_error.tex <==
\begin{figure}

  \pgfplotsset{statcorrect/.style={
      width=70mm,
      height=30mm,
      xmin=0,
      xmax=2,
      ymin=0,
      ymax=20,
      ytick={0, 5, 10, 15, 20},
      xtick={0, 0.2, ..., 2.0},
      bar width=7pt,
      ylabel near ticks,
      ylabel shift=-2pt,
      xlabel near ticks,
      ylabel style={align=center},
      %xmode=log,
      xlabel=Ratio of real error to statistical error,
      ylabel=Proportion (\%),
      legend style={
        at={(0,1.2)},anchor=south west,column sep=3pt,
        draw=none,font=\scriptsize,fill=none,font=\tiny,line width=.5pt},
      legend columns=2,
      every axis/.append style={font=\scriptsize},
      ybar=0pt,
      area legend,
  }}

  \pgfplotsset{graybar/.style={
      fill=darkteal,
      draw=none,
  }}

  \centering
  \begin{tikzpicture}
    \begin{axis}[
        statcorrect,
      ]

      \addplot[graybar]   % baseline
      table[x=x,y=y]{
        x	y
        0.05	14.29
        0.15	18.26
        0.25	12.60
        0.35	10.27
        0.45	9.73
        0.55	5.65
        0.65	8.58
        0.75	7.81
        0.85	4.21
        0.95	2.55
        1.05	1.06
        1.15	1.67
        1.25	0.99
        1.35	0.44
        1.45	0.27
        1.55	0.09
        1.65	0.31
        1.75	0.19
        1.85	0.12
        1.95	0.08
      };

    \end{axis}
  \end{tikzpicture}

  \caption{Correctness of the statistical errors produced by \dbl. The fact that
    the ratio of the real error to the statistical error is smaller than 1.0
    means that the statistical error successfully bounded the real error. For 93.9\% of
  the cases, the statistical errors were not smaller than the real errors.}
  \label{fig:exp:staterror}
  \vspace{\neggap}
\end{figure}




==> fig_model_decom_pic.tex <==
\begin{figure*}[t]

  \includegraphics[width=\textwidth]{data/fig5.png}

  %\vspace{-2mm}

  \caption{\rev{
The covariance between the answers to a pair of queries $q_i$ and $q_j$ (i.e., the
statistics we need for applying the ME principle) is equal to the
double-integration of inter-tuple covariances over respective selection predicate
ranges $\filter_i$ and $\filter_j$, due to the linearity of covariance
(equation~\ref{eq:query_cov}).}}
  \label{fig:model:decom}
  \vspace{\neggap}
\end{figure*}


==> intro_old1.tex <==
\section{Introduction}

Approximate query processing systems distinguish themselves from
traditional \emph{exact} query processing counterparts for their blazingly fast query response
times at the cost of marginal query accuracies. For example,
BlinkDB~\cite{agarwal2013blinkdb} answered queries from 7.5TB of data more than 100
times faster compared to a modern distributed database system, Hive on
Spark~\cite{engle2012shark}. These approximate database systems are becoming more
important as we live in the era of \emph{ever-growing} database sizes.

The major approach to the approximate database systems is to use \emph{database
samples} created
offline~\cite{condie2010mapreduce,acharya2000congressional,olston2009interactive,zeng2014analytical}.
When queries are submitted, those pre-generated samples (with fewer number of
tuples than an original database) are used to answer queries. The answers
computed based on the samples are \emph{approximate} because not all tuples are
used for computing answers.  However, the runtime needed to process
the sampled tuples is only a fraction of what is required to process
the entire dataset. As a result, the users of the systems can enjoy
fast response times.

In such approximate database systems, we observe an important opportunity that
has been missed in all previous works. That is, existing big database systems
spend their huge processing power to process as many database tuples in a
limited query processing time; however, all those expensive computational
efforts invested to manufacture query answers are abandoned immediately after
returning the answers to the users. On the other hand, if a database
system can characterize the relationships between past queries and a new
query, the system might be able to exploit the analyzed relationships for
improving the accuracy of new approximate query answers without accessing large
number of additional queries.

For example, suppose a following query:
\begin{lstlisting}[
  mathescape,
  basicstyle=\small\ttfamily,
  columns=fixed,basewidth=.5em,
]
    SELECT SUM(price * (1 - discount)) as revenue
    FROM sales_record
    WHERE shipdate between date '2015-01-01'
                       and date '2015-01-31'
    GROUP BY region;
\end{lstlisting}
All previous approximate systems will retrieve the tuples that satisfy the filtering
constraint (January of 2015) and compute the summation. However, if a database
system has encountered in the past the queries asking for the \texttt{revenue}
of each week of January, the system can use those answers either (1) for
answering the above query directly or (2) for improving the accuracy of the answer
that would have been returned by an existing approximate database system. In this
particular example, a system can computes an answer by summing the
revenues of all the weeks of January.

Note that reusing the past query answers provides an opportunity to increase
response speed enormously. For example, suppose 1 million tuples were processed
for computing an approximate revenue of each week of January. Then, answering
the above example query by combining these only four query answers would cost a tiny
fraction of the time needed to answer the example query without using any
of the past query answers --- the system needs to process about 4 million tuples
to achieve the same accuracy.

In this work, we generalize this idea to achieve significant query processing
speedup (or error reduction) even for complex query patterns that appear in
real-world query workloads.  Although the principle implied in the above example
might look simple on the surface, supporting more various queries in a
principled way requires more technical advances. We develop our approach based
on a robust probabilistic principle that has been widely adopted in machine
learning and statistics literature. The key property of the principle is that it
proposes what is the most best estimate based on the currently available
observations. In our case, this principle is interpreted to provide the best
answer to a new query based on the answers to past queries.

Interestingly, this probabilistic approach makes it possible to exploit past
queries even if the past queries and a new query touch exclusive areas of a
database due to their different filtering constraints. \young{Show a simple but
real example with a figure.} Our empirical experiments
show that our system can either answer approximate queries much \emph{more
accurately} for a fixed response time or can answer much \emph{more quickly} for
a fixed error constraint.




==> intro_old2.tex <==
\section{Introduction}

Approximate query processing has become an indispensable concept in many
important modern database
systems~\cite{agarwal2013blinkdb,online-agg-mr1,aqua1,dynamicp-sample-selection,chakrabarti:wavelets,ioannidis:histogram}.
When a small margin of error is permissible for query answers, approximate
database systems can return answers orders of magnitude faster than traditional
counterparts which only outputs \emph{exact} query answers.


%The performance of
%approximate database systems are improved by exploiting past queries. Past
%queries include valuable pieces of information about future queries, which is
%essentially due to the repetitive nature of database query workloads in real
%world~\cite{agarwal2013blinkdb}.

\input{intro_fig_area}

In this paper, we propose \emph{database learning}, a comprehensively novel
approach to approximate aggregate query processing. In many aspects, database learning
resembles the works in artificial intelligence: database learning makes
\emph{observations} (past queries and their answers) and \emph{learns} a model from
those observations. Moreover, database learning is a continuous process; each time a query
is processed, learning module refines the model to make it more
comprehensive\footnote{If a new query touches a data area that was not asked
before, the updated model includes information on the fresh area.}
and sophisticated\footnote{If a new query overlaps with some of past queries,
the model about the area becomes more accurate.}

In query time, database learning combines both its internal model and an answer
computed based on a sample\footnote{A sample is a subset of an entire database,
which is used to compute an approximate answer. Common approaches to sample
creation includes uniform random sampling and stratified sampling.} to
\emph{infer} a more accurate answer.  Because the internal model maintained by
the database learning is the result of all past computations, the accuracy of
the inferred answer amounts to that of the answer computed using a much larger
sample. More technically, what underpins database learning is a solid
mathematical principle, \emph{the principle of maximum
entropy}~\cite{skilling2006data}; in other words, database learning reasons
about ``what is the most likely answer given all these observations?''~by
treating database queries as random variables with a joint probability
distribution.

The idea of interpreting past queries as \emph{advice} shares some similarity with
\emph{view selection}~\cite{shukla1998materialized,gupta1997selection,agrawal2000automated,mami2012survey}
and \emph{dynamic indexing}~\cite{idreos2007database,petraki2015holistic,alagiannis2012nodb}.
However, database learning is based on a starkly different idea; thus, it results in many important distinctions:
\begin{enumerate}[noitemsep,nolistsep]
  \item Little extra storage cost: Database learning does not need large extra
    space to store indices or materialized views; it only retains past queries
    and their aggregate answers.
  \item Oblivious of data size: The size of indices and materialized views
    increase in general as data size grows. Database learning is oblivious to
    the data size growth because it only uses final aggregate answers.
  \item May accelerate even untouched data: the model learned by database
    learning often involve even the portion of the data that has been untouched
    in the past. See below for a more concrete example.
\end{enumerate}

\input{intro_fig_model}

To demonstrate database learning's behavior, suppose a following aggregate SQL query:
\begin{lstlisting}[
  mathescape,
  basicstyle=\small\ttfamily,
  columns=fixed,basewidth=.5em,
]
    SELECT AVG(price * (1 - discount)) as sales
    FROM sales_record
    WHERE shipdate between date ':from'
                       and date ':to';
\end{lstlisting}

The above SQL query asks for an average of a discounted price, and the range for
the \texttt{shipdate} may change query by query. We first generated five queries
as altering the two placeholders (\texttt{:from} and \texttt{:to}), and let
database learning process those queries. In Figure~\ref{fig:intro:model}(a), the five yellow
bars express the ranges and average values of those five aggregate queries, and
the curve in gray indicates the groundtruth average values for all data
ranges.\footnote{The curve was generated by issuing average queries with very
small range sizes and by connecting their query answers by lines.} Also, we
depicted in a red curve the model learned by database learning. In the figure,
we observe two important properties of database learning:
\begin{enumerate}[noitemsep,nolistsep]
  \item The model by database learning is accurate for the areas asked by
    queries, whereas the model does not accurately capture untapped areas.
  \item Database learning finds the best likely explanations even for the areas
    not covered by past queries. The area right from \texttt{Apr 1} and the area
    around \texttt{May 1} are such examples.
\end{enumerate}
Importantly, the database learning's ability to model the unseen areas is the
fundamental property of the maximum entropy principle. Since database
learning's inference module is based on the principle, it naturally inherits the
property. Figure~\ref{fig:intro:model}(b) illustrates the model updated after five
additional queries. Those additional queries cover some of the areas that were
not touched by the initial five queries, and the new model now has accurate
information on those areas.






==> manage.tex <==
\section{Additional Techniques}

\subsection{Incremental Update}
\label{sec:inc}

\subsection{Updating Past Queries}

As new tuples are inserted, the answers to previous queries may no longer valid,
and we may need to mark some of them invalid and discard.


==> overhead.tex <==
\section{Overhead Minimization}

Provides a formula of block matrix inversion.


==> overview_fig_workflow_pic.tex <==
%!TEX root = ldb.tex 

\begin{figure}[t]
  \centering

  \includegraphics[width=\linewidth]{data/fig2.png}

  \caption{Workflow in \dbl. At query time, the \Inference module
    improves a query answer obtained by an underlying approximate query
    processing (AQP) engine (\ie, \emph{raw
    answer}) using a \emph{Query Synopsis} and a \emph{Model}. Each time a query is processed,
    the raw query answer, \texttt{(raw ans, raw err)}, is added to the query synopsis.
    The \Learning module uses this updated query synopsis to refine the current model accordingly.
    %\young{I want to update this figure by removing Learning somehow.}
  %  \barzan{section 2 of this paper is a complete mess. Why the hell is this fig specific to \dbl ?
  %this applies to any instance of DBL, yet your entire sec 2 keeps saying \dbl. If your goal is to piss off the reviewer
  %by being messy and mix your description of DBL with \dbl then mission accomplished!}
  }
  \label{fig:overview:workflow}
  \vspace{\neggap}
\end{figure}



==> support.tex <==
\section{Advantages of Learning Database}


Describe system architecture and conditions for which our proposed techniques
can provide the best performance gains.

\begin{enumerate}[nolistsep,noitemsep]
\item Instant answers to supported aggregate queries
\item Improve the accuracy of sampling-based approximate answers
\item Natural \emph{hotspot} identification
\item No \emph{ahead-of-time} index construction
\item Full-predictive distribution and optional switch to existing methods
\item Able to use both exact and approximate answers
\end{enumerate}


